The FAST Galactic Plane Pulsar Snapshot survey: I. Project design and pulsar discoveries

Discovery of pulsars is one of the main goals for large radio telescopes. The Five-hundred-meter Aperture Spherical radio Telescope (FAST), that incorporates an L-band 19-beam receiver with a system temperature of about 20~K, is the most sensitive radio telescope utilized for discovering pulsars. We designed the {\it snapshot} observation mode for a FAST key science project, the Galactic Plane Pulsar Snapshot (GPPS) survey, in which every four nearby pointings can observe {\it a cover} of a sky patch of 0.1575 square degrees through beam-switching of the L-band 19-beam receiver. The integration time for each pointing is 300 seconds so that the GPPS observations for a cover can be made in 21 minutes. The goal of the GPPS survey is to discover pulsars within the Galactic latitude of $\pm10^{\circ}$ from the Galactic plane, and the highest priority is given to the inner Galaxy within $\pm5^{\circ}$. Up to now, the GPPS survey has discovered 201 pulsars, including currently the faintest pulsars which cannot be detected by other telescopes, pulsars with extremely high dispersion measures (DMs) which challenge the currently widely used models for the Galactic electron density distribution, pulsars coincident with supernova remnants, 40 millisecond pulsars, 16 binary pulsars, some nulling and mode-changing pulsars and rotating radio transients (RRATs). The follow-up observations for confirmation of new pulsars have polarization-signals recorded for polarization profiles of the pulsars. Re-detection of previously known pulsars in the survey data also leads to significant improvements in parameters for 64 pulsars. The GPPS survey discoveries are published and will be updated at http://zmtt.bao.ac.cn/GPPS/ .

==> known64psr_table.tex <==
\begin{table*}
  \centering
  
  \begin{minipage}{9cm}
  \caption{Some Parameters are Updated for 64 Known Pulsars}
  \label{para64psr}\end{minipage}
  
  \fns
  \tabcolsep 0.7mm
  \begin{tabular}{lllrllclcrcc}
    \hline
PSR name      & Ref. & P in Ref. & DM  &  RA(2000)    &  \multicolumn{1}{c}{Dec(2000)}    & Updated &  \multicolumn{1}{c}{P ($\sigma$)} & Epoach for P  & DM ($\sigma$) &  RA(2000) &  Dec(2000)  \\
&      & \multicolumn{1}{c}{(s)} &  & hh:mm:ss.s & \multicolumn{1}{c}{dd:mm:ss}& items & \multicolumn{1}{c}{(s) }   &   (MJD)   &  & hh:mm:ss.s &\multicolumn{1}{c}{dd:mm} \\
(1) & (2) & \multicolumn{1}{c}{(3)} & (4) &\multicolumn{1}{c}{ (5)} & \multicolumn{1}{c}{ (6)} & (7) &\multicolumn{1}{c}{ (8)} & (9) &\multicolumn{1}{c}{ (10)} & (11) & (12)  \\
 \hline
J0611+1436  &    [1]      &  0.270329   &  45.7    &  06:11:18.65   &  +14:36:52     &  DM     &  0.27032969(38)   &  58847.665398  &  43.7(2)    &  06:11:17  &  +14:37    \\
J0658+0022  &    [2]      &  0.563295   &  122.0   &  06:58:15.21   &  +00:22:35.3   &  DM     &  0.5632972(16)    &  58839.756478  &  115.6(5)   &  06:58:14  &  +00:23    \\
J1832+0029  &    [3]      &  0.533917   &  28.3    &  18:32:50.7    &  +00:29:27     &  DM     &  0.5339170(16)    &  58765.445867  &  32.7(4)    &  18:32:48  &  +00:30    \\
J1843+01    &    [8]      &  1.26702    &  248.0   &  18:43         &  +01           &  Posi   &  1.266990(12)     &  59198.252593  &  251.9(16)  &  18:43:28  &  +01:19    \\
J1847+01    &    [4]      &  0.00346    &  20.0    &  18:47         &  +01           &  Posi   &  0.0034630711(1)  &  59093.545385  &  20.100(5)  &  18:47:05  &  +01:13    \\
J1848-0023  &    [5]      &  0.537624   &  30.6    &  18:48:37.89   &  $-$00:23:17   &  DM     &  0.53762431(52)   &  59077.578982  &  34.6(4)    &  18:48:40  &  $-$00:24  \\
J1849+01    &    [4]      &  1.832      &  213.6   &  18:49         &  +01           &  Posi   &  1.832250(18)     &  58909.025657  &  217.2(15)  &  18:49:56  &  +01:06    \\
J1849+0409  &    [3]      &  0.761194   &  56.1    &  18:49:3.47    &  +04:09:42.3   &  DM     &  0.7612033(32)    &  58720.600254  &  64.1(6)    &  18:49:03  &  +04:09    \\
J1849+04    &    [4]      &  0.42111    &  191.8   &  18:49         &  +04           &  Posi   &  0.4211266(11)    &  58720.585427  &  188.2(4)   &  18:49:40  &  +04:30    \\
J1849-0040  &    [5]      &  0.672481   &  1234.9  &  18:49:10.25   &  $-$00:40:20   &  DM     &  0.672479(8)      &  59244.140909  &  1267.6(18) &  18:49:11  &  $-$00:40  \\
J1850-0006  &    [6]      &  2.191498   &  570.0   &  18:50:47.93   &  $-$00:06:26.1 &  DM     &  2.1915070(88)    &  59082.572228  &  655.0(18)  &  18:50:47  &  $-$00:07  \\
J1851+00    &    [4]      &  0.02283    &  107.4   &  18:51         &  +00           &  Posi   &  0.0228466631(27) &  58902.066301  &  107.60(2)  &  18:51:02  &  +00:10    \\
J1851+0242  &    [4]      &  1.49714    &  534.1   &  18:51:22      &  +02:42:37     &  P      &  4.4912(2)        &  58997.792192  &  519.3(71)  &  18:51:19  &  +02:42    \\
J1852+00    &    [4]      &  1.92066    &  590.4   &  18:52         &  +00           &  Posi   &  1.920653(21)     &  58923.007492  &  590.0(15)  &  18:52:39  &  +00:00    \\
J1853+0009  &    [4]      &  0.03341    &  192.0   &  18:53         &  +00:09        &  Posi   &  0.033395062(2)   &  58939.971197  &  192.40(3)  &  18:53:39  &  +00:08    \\
J1853+0029  &    [4]      &  0.93832    &  230.0   &  18:53         &  +00:29        &  Posi,P &  1.8767568(63)    &  59112.477816  &  227.1(15)  &  18:53:18  &  +00:29    \\
J1853+03    &    [7]      &  0.58553    &  290.2   &  18:53         &  +03:00        &  Posi   &  0.5855545(32)    &  58977.860290  &  295.8(8)   &  18:53:12  &  +03:00    \\
J1853+04    &    [8]      &  1.32065    &  549.3   &  18:53         &  +04           &  Posi   &  1.320623(13)     &  59004.780117  &  548.9(13)  &  18:53:46  &  +04:27    \\
J1854+00    &    [7]      &  0.76733    &  532.9   &  18:54         &  +00:00        &  Posi   &  0.767278(1)      &  58940.968884  &  525.0(6)   &  18:54:43  &  +00:50    \\
J1854+0317  &    [9]      &  1.36645    &  404.0   &  18:54:29.06   &  +03:17:31     &  DM     &  1.366465(11)     &  58991.813118  &  390.0(11)  &  18:54:29  &  +03:17    \\
J1855+0422  &    [10]     &  1.678106   &  438.0   &  18:55:41.37   &  +04:22:47     &  DM     &  1.678105(15)     &  59187.292726  &  455.6(13)  &  18:55:41  &  +04:22    \\
J1858+02    &    [7]      &  0.19765    &  492.1   &  18:58         &  +02:00        &  Posi   &  0.19764740(24)   &  58900.051935  &  492.8(2)   &  18:58:23  &  +02:41    \\
J1853+0853  &    [3]      &  3.914658   &  214.0   &  18:53:22.07   &  +08:53:17     &  DM     &  3.914696(79)     &  59253.091997  &  236.6(31)  &  18:53:20  &  +08:54    \\
J1859+00    &    [11],[5] &  0.559634   &  420.0   &  18:59:46      &  +00:35        &  Posi   &  0.5596363(18)    &  58982.867548  &  424.0(4)   &  18:59:47  &  +00:38    \\
J1859+03    &    [4]      &  1.51171    &  555.1   &  18:59         &  +03           &  Posi   &  1.511506(28)     &  58867.217455  &  558.7(26)  &  18:59:10  &  +03:46    \\
J1901+00    &    [11],[5] &  0.777662   &  345.5   &  19:01:32      &  +00:26        &  Posi   &  0.7776620(32)    &  58977.880799  &  340.3(6)   &  19:01:32  &  +00:32    \\
J1901+0435  &    [3]      &  0.690576   &  1042.6  &  19:01:32.2    &  +04:35:23     &  DM     &  0.690605(11)     &  58565.032593  &  920.0(25)  &  19:01:31  &  +04:35    \\
J1902+02    &    [7]      &  0.41532    &  281.2   &  19:02         &  +02:00        &  Posi   &  0.4153927(11)    &  59233.161342  &  280.4(4)   &  19:02:31  &  +02:35    \\
J1903+0415  &    [7]      &  1.15139    &  473.5   &  19:03         &  +04:15        &  Posi   &  1.151411(11)     &  58902.108022  &  481.9(14)  &  19:03:30  &  +04:15    \\
J1903+09    &    [4]      &  0.16631    &  362.9   &  19:03         &  +09           &  Posi   &  0.16631690(28)   &  59164.332493  &  362.9(3)   &  19:03:39  &  +09:12    \\
J1905+10    &    [4]      &  1.72688    &  165.7   &  19:05         &  +10           &  Posi   &  1.726813(17)     &  58852.191366  &  163.7(14)  &  19:05:19  &  +10:34    \\
J1906+0725  &    [7]      &  1.53651    &  480.4   &  19:06         &  +07:25        &  Posi   &  1.536442(14)     &  58770.485688  &  476.4(12)  &  19:06:23  &  +07:25    \\
J1907+05    &    [7]      &  0.16868    &  456.7   &  19:07         &  +05:00        &  Posi   &  0.16867706(35)   &  58982.878143  &  457.1(3)   &  19:08:02  &  +05:59    \\
J1909+12    &    [4]      &  1.229338   &  292.5   &  19:09:57.7    &  +12:04:55.3   &  DM     &  1.229319(8)      &  59189.269571  &  302.5(10)  &  19:09:51  &  +12:06    \\
J1910+1027  &    [7]      &  0.53147    &  705.7   &  19:10         &  +10:27        &  Posi   &  0.5315526(26)    &  59093.531512  &  715.3(7)   &  19:10:48  &  +10:27    \\
J1910+07    &    [4]      &  0.53869    &  256.5   &  19:10         &  +07           &  Posi   &  0.5386463(54)    &  58911.070131  &  255.3(15)  &  19:10:06  &  +07:11    \\
J1911+09    &    [7]      &  0.27371    &  334.7   &  19:11         &  +09:00        &  Posi   &  0.27370588(47)   &  59067.582251  &  340.7(8)   &  19:11:47  &  +09:22    \\
J1911+10    &    [7]      &  0.19089    &  446.2   &  19:11         &  +10:00        &  Posi   &  0.19087553(57)   &  59155.408562  &  445.0(5)   &  19:11:43  &  +10:52    \\
J1913+05    &    [4]      &  0.662      &  330.1   &  19:13         &  +05           &  Posi   &  0.6619994(40)    &  59185.290377  &  335.9(9)   &  19:13:22  &  +05:24    \\
J1914+08    &    [12]     &  0.440048   &  285.0   &  19:14:18      &  +08:45        &  Posi   &  0.44003996(35)   &  59090.587469  &  290.6(4)   &  19:14:25  &  +08:39    \\
J1916+1023  &    [5]      &  1.618339   &  329.8   &  19:16:36.91   &  +10:23:03     &  DM     &  1.618330(14)     &  58909.104157  &  341.8(13)  &  19:16:37  &  +10:23    \\
J1918+1541  &    [13]     &  0.370883   &  13.0    &  19:18:7.7     &  +15:41:15.2   &  DM     &  0.37088498(71)   &  59198.231761  &  11.4(3)    &  19:18:10  &  +15:42    \\
J1920+1110  &    [10]     &  0.509886   &  182.0   &  19:20:13.31   &  +11:10:59     &  DM     &  0.5098862(16)    &  58977.910791  &  188.4(4)   &  19:20:14  &  +11:11    \\
J1924+1628  &    [7]      &  0.37509    &  542.9   &  19:24         &  +16:28        &  Posi   &  0.37508191(88)   &  58808.402942  &  541.7(3)   &  19:24:45  &  +16:29    \\
J1924+17    &    [7]      &  0.75843    &  527.4   &  19:24         &  +17:00        &  Posi   &  0.7584369(11)    &  59069.686122  &  540.9(7)   &  19:24:32  &  +17:14    \\
J1924+2040  &    [14],[15]&  0.23779    &  213.0   &  19:24:40      &  +20:40:03     &  DM     &  0.2377930(3)     &  58843.315936  &  226.6(2)   &  19:24:35  &  +20:40    \\
J1926+1613  &    [7]      &  0.3083     &  32.9    &  19:26         &  +16:13        &  DM,Posi&  0.308304(1)      &  58936.061255  &  24.5(5)    &  19:26:51  &  +16:14    \\
J1927+1852  &    [16]     &  0.482766   &  254.0   &  19:27:10.42   &  +18:52:8.5    &  DM     &  0.48276601(42)   &  58940.066550  &  264.5(4)   &  19:27:07  &  +18:51    \\
J1929+1905  &    [17]     &  0.339243   &  553.9   &  19:29:31.7    &  +19:05:43.4   &  DM     &  0.33921584(21)   &  59174.390702  &  528.4(3)   &  19:29:14  &  +19:10    \\
J1930+14    &    [7]      &  0.42571    &  209.2   &  19:30         &  +14:00        &  Posi   &  0.4257200(22)    &  58808.383858  &  214.8(7)   &  19:30:19  &  +14:09    \\
J1930+17    &    [18]     &  1.60969    &  201.0   &  19:30:44      &  +17:25        &  Posi   &  1.609723(13)     &  59157.422738  &  197.4(13)  &  19:30:31  &  +17:23    \\
J1934+19    &    [7]      &  0.23099    &  97.6    &  19:34         &  +19:00        &  Posi   &  0.23098462(95)   &  58995.887279  &  98.4(5)    &  19:34:18  &  +19:26    \\
J1936+18    &    [4]      &  0.05835    &  125.5   &  19:36         &  +18           &  Posi   &  0.05834513(18)   &  58997.893701  &  125.9(4)   &  19:36:03  &  +18:05    \\
J1936+20    &    [7]      &  1.39088    &  205.1   &  19:36         &  +20:00        &  DM,Posi&  1.3907326(35)    &  59102.591721  &  195.9(11)  &  19:36:29  &  +20:41    \\
J1936+21    &    [18]     &  0.642932   &  264.0   &  19:36:29      &  +21:12        &  Posi   &  0.6429599(22)    &  58944.052936  &  262.4(5)   &  19:36:11  &  +21:09    \\
J1936+21a   &    [4]      &  0.0316     &  73.9    &  19:36         &  +21           &  Posi   &  0.03158187(3)    &  59155.467443  &  75.0(2)    &  19:37:00  &  +21:43    \\
J1938+14    &    [19]     &  2.90251    &  74.2    &  19:38:19      &  +14:42        &  Posi   &  2.902504(51)     &  59209.202485  &  75.4(23)   &  19:38:07  &  +15:06    \\
J1939+26    &    [4]      &  0.46593$*$ &  48.1    &  19:39         &  +26           &  Posi   &  0.4669615(11)    &  59253.183278  &  47.5(4)    &  19:39:42  &  +26:09    \\
J1940+26    &    [4]      &  0.00481    &  171.6   &  19:40         &  +26           &  Posi   &  0.0048135292(14) &  59253.175813  &  171.61(4)  &  19:40:13  &  +26:01    \\
J1955+29    &    [4]      &  1.07377    &  206.0   &  19:55         &  +29           &  Posi   &  1.0738820(62)    &  58735.618100  &  212.4(9)   &  19:55:07  &  +29:31    \\
J2000+29    &    [8]      &  3.0737     &  132.5   &  20:00         &  +29           &  Posi   &  3.073809(58)     &  58901.180519  &  131.3(25)  &  20:00:14  &  +29:21    \\
J2003+29    &    [4]      &  1.00987    &  208.7   &  20:03         &  +29           &  Posi   &  1.0098800(56)    &  58943.068686  &  209.5(8)   &  20:03:02  &  +29:16    \\
J2010+31    &    [4]      &  1.55147    &  251.0   &  20:10         &  +31           &  Posi   &  1.551535(24)     &  58910.171365  &  251.8(23)  &  20:10:35  &  +31:50    \\
J2138+4911  &    [20]     &  0.696      &  168.0   &  21:38         &  +49:11        &  Posi   &  0.696171(3)      &  58941.118314  &  168.0(6)   &  21:38:15  &  +49:12    \\
\hline\noalign{\smallskip}
 \end{tabular}
 
\parbox{17cm}{(1) Reference in Column~(2): 
[1]: \citet{lyne2017};
[2]: \citet{Burgay2013};
[3]: \citet{Lorimer2006};
[4]: {\it \url{http://www.naic.edu/~palfa/newpulsars/}}; 
[5]: \citet{hfs+04};
[6]: \citet{kel+09};
[7]: \citet{lbh+15};
[8]: \citet{patel2018};
[9]: \citet{Eatough2013};
[10]: \citet{mhl+02}; 
[11]: \citet{camilo1996}
[12]: \citet{kbj+18};
[13]: \citet{Camilo1995};
[14]: \citet{Weisberg1981};
[15]: \citet{vms83}; 
[16]: \citet{Lorimer2002};
[17]: {\it\url{http://astro.phys.wvu.edu/dmb/}};
[18]: \citet{Lorimer2013};
[19]: \citet{Deneva2016};
[20]: \citet{Hessels2008}.  \\
  (2) Columns (3)--(6) are parameters in the reference, and
  Columns~(7), (9), (10) and (11) are paramters obtained in the GPPS survey; \\  
   DM has a unit of cm$^{-3}$~pc. Newly measured P and DM have an uncertainty in brackets. $*$: mistyping in the reference.} 
\end{table*}

